Agujeros Negros con Pelo y Dualidad AdS/CFT

The present thesis is based in the material previously published in [arXiv:1501.04252, arXiv:1511.08759, arXiv:1606.07870] and it is organized in the following way. The second chapter is shown as the isometric group of the space time AdS is exactly (isomorphic) match to the conformal group of the dual CFT theory. We present the precise formulation of the duality AdS/CFT and we describe the behavior of a massive scalar field in AdS space-time. In chapter 3 we present solutions of black holes widely known in the literature, which we will use in some later calculations to gain intuition, we explain the no-hair theorem and two examples of exact black hole solutions that can evade this theorem. These results were published in [arXiv:1211.2765, arXiv:1311.6065, arXiv:1311.7459]. Chapter 4 we present details of the methods of holographic renormalization and Hamiltonian formalism, which are applied in the development of the later chapters. For the solution SAdS calculate the on-shell action and regularize, compare with the method of subtraction of the background. Chapter 5 is based on [arXiv:1606.07870]. We investigated the boundary conditions of AdS in the presence of a scalar field minimally coupled to gravity with conformal mass $m^{2}=-2/l^{2}$, for non-logarithmic and logarithmic branch. We calculate the on-shell action, we study the variational principle and propose new counter-terms that regularize the action. Chapter 6, is based on [arXiv:1501.04252, arXiv:1606.07870], we describe the phase transitions of black holes with scalar hair and horizons flat and spherical. We build the thermodynamic phase diagrams and discuss their implications in the dual quantum field theory. Finally in chapter 7 the conclusions and future directions of the work are presented.

==> titlepage.tex <==
%% ## Construye tu propia portada ##
%% 
%% Una portada se conforma por una secuencia de "Blocks" que incluyen
%% piezas individuales de informaci'on. Un "Block" puede incluir, por
%% ejemplo, el t'itulo del documento, una im'agen (logotipo de la universidad),
%% el nombre del autor, nombre del supervisor, u cualquier otra pieza de
%% informaci'on.
%%
%% Cada "Block" aparece centrado horizontalmente en la p'agina y,
%% verticalmente, todos los "Blocks" se distruyen de manera uniforme 
%% a lo largo de p'agina.
%%
%% Nota tambi'en que, dentro de un mismo "Block" se pueden cortar
%% lineas usando el comando \\
%%
%% El tama'no del texto dentro de un "Block" se puede modificar usando uno de
%% los comandos:
%%   \small      \LARGE
%%   \large      \huge
%%   \Large      \Huge
%%
%% Y el tipo de letra se puede modificar usando:
%%   \bfseries - negritas
%%   \itshape  - it'alicas
%%   \scshape  - small caps
%%   \slshape  - slanted
%%   \sffamily - sans serif
%%
%% Para producir plantillas generales, la informaci'on que ha sido inclu'ida
%% en el archivo principal "tesis.tex" se puede accesar aqu'i usando:
%%   \insertauthor
%%   \inserttitle
%%   \insertsupervisor
%%   \insertinstitution
%%   \insertdegree
%%   \insertfaculty
%%   \insertdepartment
%%   \insertsubmitdate

%%%%%%%%%%%%%%%%%%PORTADA%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%escudo_uni
\begin{titlepage}
  \TitleBlock{\includegraphics[height=3.5cm]{insignia.eps}  \\
  \scshape\insertinstitution}
%  \vspace*{3cm}
 % \TitleBlock[\bigskip]{\scshape\insertfaculty}
   \TitleBlock[\vspace*{3cm}]   
  \TitleBlock{\Huge\scshape\inserttitle}
  \TitleBlock{\scshape
    Tesis presentada por \insertauthor \\
    para obtener el grado de \insertdegree}
   
  \TitleBlock{\small\scshape
    \insertsupervisor}   
    
  \TitleBlock{NOVIEMBRE 2016}
  \TitleBlock[\bigskip]{\insertdepartment}
\end{titlepage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}
%%%pagina en blanco%%%%
\end{titlepage}

%%%%%%%%%%COMITE EXAMINADOR%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%FIRMAS%%%%%%%%%%%%%%%%%%%

\begin{titlepage}

\begin{flushleft}
TITULO DE TESIS:\\
\TitleBlock{\huge\scshape\inserttitle}
\end{flushleft}


\begin{flushleft}
AUTOR:\\
\TitleBlock{\scshape\insertauthor}
\end{flushleft}

\TitleBlock[\vspace*{1cm}]

  \TitleBlock{\scshape
    Tesis presentada por \insertauthor \\
    para obtener el grado de \insertdegree}

\begin{flushleft}
\TitleBlock{\scshape COMITE EXAMINADOR:}
\end{flushleft}

\begin{flushleft}
\TitleBlock{\scshape Dr. Dumitru Astefanesei \hspace{0.7cm} (PUCV) ............................................}
\end{flushleft}

\begin{flushleft}
\TitleBlock{\scshape Dr. Andr\'es Ace\~na \hspace{2.5cm} (UC) ................................................}
\end{flushleft}

\begin{flushleft}
	\TitleBlock{\scshape Dr. Olivera Mi\v skov\'ic \hspace{1.5cm} (PUCV) .............................................}
\end{flushleft}

\begin{flushleft}
\TitleBlock{\scshape Dr. Alfonso Zerwekh  \hspace{1.5cm} (UTFSM) ..........................................}
\end{flushleft}

\TitleBlock[\vspace*{0.5cm}]

\begin{flushright}
\TitleBlock{\small\scshape\ Valpara\'iso, Chile. Noviembre 16, 2016}
\end{flushright}


\end{titlepage}


%% Nota 1:
%% Se puede agregar un escudo o logotipo en un "Block" como:
%%   \TitleBlock{\includegraphics[height=4cm]{escudo_uni}}
%% y teniendo un archivo "escudo_uni.pdf", "escudo_uni.png" o "escudo_uni.jpg"
%% en alg'un lugar donde LaTeX lo pueda encontrar.

%% Nota 2:
%% Normalmente, el espacio entre "Blocks" se extiende de modo que el
%% contenido se reparte uniformemente sobre toda la p'agina. Este
%% comportamiento se puede modificar para mantener fijo, por ejemplo, el
%% espacio entre un par de "Blocks". Escribiendo:
%%   \TitleBlock{Bloque 1}
%%   \TitleBlock[\bigskip]{Bloque2}
%% se deja un espacio "grande" y de tama~no fijo entre el bloque 1 y 2.
%% Adem'as de \bigskip est'an tambi'en \smallskip y \medskip. Si necesitas
%% aun m'as control puedes usar tambi'en, por ejemplo, \vspace*{2cm}.



